PIPS, an advanced platform for period detection in time series -- I. Fourier-likelihood periodogram and application to RR Lyrae Stars

We describe the $\texttt{Period detection and Identification Pipeline Suite}$ ($\texttt{PIPS}$) -- a new, fast, and statistically robust platform for period detection and analysis of astrophysical time-series data. $\texttt{PIPS}$ is an open-source Python package that provides various pre-implemented methods and a customisable framework for automated, robust period measurements with principled uncertainties and statistical significance calculations. In addition to detailing the general algorithm that underlies $\texttt{PIPS}$, this paper discusses one of $\texttt{PIPS'}$ central and novel features, the Fourier-likelihood periodogram, and compares its performance to existing methods. The resulting improved performance implies that one can construct deeper, larger, and more reliable sets of derived properties from various observations, including all-sky surveys. We present a comprehensive validation of $\texttt{PIPS}$ against artificially generated data, which demonstrates the reliable performance of our algorithm for a class of periodic variable stars (RR Lyrae stars).

==> extra/classification.tex <==
\section{Classification Algorithm}
    \label{sec:classification_algorithm}
    The classifier included in \PIPS is based on the random forest (RF) classification algorithm \citep{Ho1995_RF}, which itself relies on the decision tree (D-Tree) algorithm. D-Trees and RFs have been used for numerous classification tasks on various datasets with considerable success \citep{Hinners2018_MLexoplanet,Ball2010_MLreview}. 
    The D-Tree algorithm works by hierarchically splitting the data, based on the given features, into subsets for each class such that each subset is maximally mutually dissimilar, while achieving most similarity within each group. This criterion of similarity is quantified by metrics such as the Gini index and entropy, which are the cost functions used to optimise the classifier \citep{derosa2016_gini}.
    The RF algorithm is an improvement upon the D-Tree classifier that randomly resamples the training data and creates multiple decision trees for these samples in a process known as bootstrapping. Each D-Tree uses a different, randomly chosen hierarchy of feature nodes (i.e., order of splitting) and makes its own decision on the classification. In the end, all the trees vote on the outcome, and the class with a plurality of votes is assigned to the data being classified \citep{Sarica2017_MLpubmed}.

    We use the RF classifier implemented in the \texttt{scikit-learn} Python package \citep[][]{scikit-learn}. 121,907 stars in total (10,281 classical Cepheids, 1856 Type~II Cepheids, 88,411 RRab stars, and 21,359 RRc stars) are extracted from the OGLE variable-star database \citep{udalski2015_ogleiv,udalski2008ogle_iii} to develop the algorithm. 900 stars from each class are then chosen as our training data, and the rest are earmarked as testing data to determine the accuracy of the model on the preclassified data. This is done to ensure that no bias is introduced owing to any mismatch in the sizes of the training data of the different classes.
    The OGLE database contains data on the stars' periods and the Fourier parameters. The model is trained on these data using the period and the $r_{21}$, $r_{31}$, $\phi_{21}$, and $\phi_{31}$ parameters. A 100-tree RF is used with a depth of 10. The model returns 99\% training accuracy. Upon deploying this model on the held-out testing data, the model returns a 98\%  accuracy score.

    To further test the validity of this model, we use the {\it Gaia} variable-star database \citep{gaia2016_main,gaia2018dr2,GaiaDR2_variability} as an additional testing set. Since these data were obtained from a completely different, independently compiled source, a good test score on them would make a strong case that the model is not biased toward the OGLE data sample used to train it. After removing objects that have missing information, we obtain 271 classical Cepheids, 43 Type~II Cepheids, 910 RRab stars, and 445 RRc stars in our {\it Gaia} testing set. Upon running the algorithm on these data, we obtain a 94\% testing accuracy, suggesting that the model is not biased toward OGLE data and is indeed applicable across datasets.

